Component-Wise Boosting of Targets for Multi-Output Prediction

Multi-output prediction deals with the prediction of several targets of possibly diverse types. One way to address this problem is the so called problem transformation method. This method is often used in multi-label learning, but can also be used for multi-output prediction due to its generality and simplicity. In this paper, we introduce an algorithm that uses the problem transformation method for multi-output prediction, while simultaneously learning the dependencies between target variables in a sparse and interpretable manner. In a first step, predictions are obtained for each target individually. Target dependencies are then learned via a component-wise boosting approach. We compare our new method with similar approaches in a benchmark using multi-label, multivariate regression and mixed-type datasets.

==> latex-math/.git/objects/48/ec0d3c3f39979e6b39721d98322c6e4b6199db <==
x}RËjÃ0ì9_±L4"ôPh½†Òk NÙ^W&¶åJ²+#ôï]5ÐÆÊÁwwfgf"R$ð¼|º‹ *ao¯ï£¸ÆïTT«3+ݍ9ÓV¹©™9ˆ ­S"šµîAQ…~gº"™Ý£ŸÖ+¦WJOr»rAù 4"æ¿áà>æç ¦)Üf¹Ý[kvv>/g!PÇ=
Öª•èÉH
§}bÓÍ\lTÃRtð÷EPŠ"•€JԍtLŒÄÓÐÒf(D] ¸ä\HpêäuŽ@Ã1‹¼'›Ãå›ÐœD"™ê+z¬q»yè&~µB£÷Üî÷ãådÄÖaz1Äëƒî~{ˆ³ׁ~Ÿ$åd×î'd¢¢Û"PÈdÊá7çÑ(VJdYæEMñRSÂT'.<â5¿ïˆ÷Ē>Ü???ç·Â§+"â"è˜ï!A­QB«âŠȅ"FbV¤ÇÓ+[ü°UÝ

==> latex-math/.git/objects/59/78fc6c17236da0aff0e38a321d0339046fd290 <==
xÎMŠ1@a×9Eí$?•ØqösaHUª´Ñn%"a<¾=Áå[<øø6McÃª7pbÐ
Z.h#åê"ó˜©
–˜½«êÔÜK"y–èÔ'VOCÅ\%K,V´ÉI‡r&S~ûùÖà m®pø|…-ý×7½jšëYú\DRLèáÃzk
¿]ÞÜÍ"•?à©BmÂÐrü'²HŽŸæ	¯Os

==> latex-math/.git/objects/74/6310438549b5d8042754ce038c7327268a925c <==
xŽ;Â0©}ŠíÈvðOBJŽ±»^"HĆ`NO
N@÷4Òh·yž:Ø!nú"†óI—2›\9$'hµÖ\'
YlT\¤v0t ï‹6CR*Îì¢K&e#9Z¯ðÝǶÀkÄû¸»\áøÛûÏó|›qºï¹Í'0nH«cò°ÕkS­t½Øå/Yað51Ô
µuìS«ê*UL

==> latex-math/.git/objects/ab/32856893ac75fd4ce2f18b72cd2c1e3525fb71 <==
x¥WmoÛ6ÞWëWh1ͨ³bÀ€m@àH>ÔyY±©º''(›¨H
$åÈôßw¤å*Ja¥bG4ï¹÷çÎI!øù×÷¿ü'fº$)ÕAÌòŒæLÐ,^Àw¾BXD ˆ©)YQAŸRÉ9Y/Ú&¶Š³fѶc!2tfB²3Í*ÁL}ožV,]Á…JÓ·äRÁÙâ꟏·‹³ ¦…¦@<h‡~…!Aœ³'¶žöÇ]tó8>ÂcLº¤
#|ì×ýùþUÈ÷(b˜.yÇÐè‡WA? 4u°‡j›ÛÄø%2?虏ÔÂ<¬µ² õpÞGƒw®¯ÿêüIIÑ\t0×׬X'Pe\³úùN¥0LT²ÒGZN›˜ƒ™cäv`W"µUÐ+¯GZ> /"£—e"t…¢âhnO"–š£4~°BŠ/ü¹pÍxŁ*%U!$D³´£)Så¹ïymÍ°"£P·GfL&!Ôà¾bd‹˜¨%'õ–vdÙÄ:<Š#<"ÐJ¡Ì"‰P&ƃ2ỦÙR s²¤ØŠR	ÂiãÎNcÌìåȽW܇¾é˜$ÍÍC;ºáÆ2OÆRk˜-UFUokýv~·86/ÛOŸ›8W$mâ'(ÃHç3Ô´¸xYU»[h[#µ­©¯ Ì4¨ §a[cƒxX¬ºâpÄA©dV¥¦Wýø5V_Å¿4ì÷Yû¯8.Z's;r%9à0ú…Qñ¯ËÊW‹²ü&
^±(˞Ãh¡3ƚ:lMçÄ·l±Wœ1["!k<"½-¬Y'( Œ&ŠøÖIAÑÃD™Þpüh0#†m³ìZ°¦é³ý*iÁyó®=œåŒw?
I°Ì7æM³í™Œ"·šïkƈM§×èîì4C°—#÷n¶n°al(=t£NfFEø‡ >®.Ÿ"SIN¦=,u¼ÝƒL»&/hn₈eA±Å#8¿Àí€-W&Vîp8.!ü6¦ ã!ïՕ¯›«ý4ûÜx#Ëæ]¯¤2Pâ÷ŠÕvy°‹j0‰ºD'ïÎÛ`29Ÿá)Å%vÖú*.­W]—Ϫ«ƒ¿ô%êõö>¢ÞÛÖ"²7¶Þúb›Nló'ØfPìOZ'l5ÆîÁ"·£UÜmÐ[4ºî½£"X×ð#hC,ëùËܪCßW™nîN­¼}·‡pY>Ý)ñ£pu€¾
m««h]"M8ÞõÁ×d7ÊtÞüÕ·7µ÷O(¢0"ú
"J›?ĞãÃXl"±kîKèêÈô¹Ä§1ø¸¢ˆ…WŠ'RqRtØ9?ý
‡«¦Yášè½4¶^RÙáç'9ö•kÜ%©iؔM-kÆOóÈÒ£6ðÄðw®Æ!+•N+¯É^$ÚD¼ÓçVŒÓ"…0Néƒ/4¢Ýið?À8Z

==> latex-math/chapter-notation.tex <==
\section{General Notation and Terminology}
\label{sec:notation}

Consider a $p-$dimensional feature space $\Xspace = (\Xspace[1] \times \Xspace[2] \times \hdots \times \Xspace[p])$ %of arbitrary measurement scales
and a target space $\Yspace$.
Suppose that there is an unknown functional relationship $f$ between $\Xspace$ and $\Yspace$.
ML algorithms try to learn this relationship using training data with observations that have been drawn i.i.d. from an unknown probability distribution $\mathcal{P}$ on the joint space $\Xspace \times \Yspace$.
%The learned prediction model will be denoted by $\fh$ and approximates $f$.
We consider an arbitrary prediction model $\fh$, fitted on some training data to approximate $f$ and analyze it with model-agnostic interpretability methods.
Let $\D = \Dset$ be a test data set sampled i.i.d. from $\mathcal{P}$ where $n$ is the number of observations in the test set.
Let $P = \{1, \hdots, p\}$ be an index set referring to all features.
We denote the corresponding random variables generated from the feature space by $X = (X_1, \hdots, X_p)$ and the random variable generated from the target space by $Y$.
In our notation, the vector $\xi = \xivec \in \Xspace$ refers to the $i$-th observation which is associated with the target outcome $\yi \in \Yspace$ and $\xj = \xjvec$ denotes the realizations of the $j$-th feature.
%Suppose that there is an unknown functional relationship $f$ that maps each observation $\xi$ to its target outcome $\yi$.
% Performane estimation
% The performance estimation of a ML algorithm is based on training the algorithm on training data and estimating the \emph{generalization error} (also known as \emph{test error}) of the algorithm on new (unseen) test data.
We denote the generalization error of a fitted model on unseen test data from $\mathcal{P}$ by $GE(\fh, \mathcal{P}) = \E(L(\fh(X), Y))$, measured by a loss function $L$.
%with which the performance of $\fhD$ is measured.
It can be estimated using the test data $\D$ by %through the empirical expected loss
%by splitting the observed data $\D$ into a training set $\Dtrain$ and test set $\Dtest = \D \setminus \Dtrain$, fitting the model on the training set and averaging the loss or gain function over an independent test set using
\begin{equation}
\label{eq:geest}
%\GEh{}(\fh, \D) = \frac{1}{|\D|} \sum_{\xy \in \D} L(\fh(x), y).
\textstyle \GEh{}(\fh, \D) = \frac 1 n \sum_{i=1}^n \Lii.
\end{equation}
%Note that if $\fh$ was trained on $\D$ and if the generalization error uses again $\D$ to measure the performance, we obtain an estimate for the training error.
%We therefore consider $\fh$ as a fixed model that was trained on $\Dtrain$ which is i.i.d. from $\D$. %the observations from the data set $\D$ were not used to fit the model $\fh$.
A better estimate for the generalization error of an ML algorithm can be obtained using resampling techniques such as cross-validation or bootstrap \citep{Bischl2012}. %as they %reuse the observed data at hand to produce a better estimator.
%Specifically, they repeatedly split the observed data into training and test sets of equal size, fit a model using the produced training sets and estimate the performance on the remaining test sets.
%The resulting performance values on each test set are then aggregated by averaging in order to estimate the generalization error more precisely \citep[see e.g.][]{Bischl2012}.


==> latex-math/ml-bagging.tex <==
% ml - bagging, random forest

\newcommand{\bl}[1]{b^{[#1]}(x)}											% baselearner with argument for m
\newcommand{\blm}{\bl{m}}												    % baselearner without argument for m
\newcommand{\blmh}{\hat{b}^{[m]}(x)}										% estimated base learner 
\newcommand{\fM}{f^{[M]}(x)}                    % ensembled predictor


==> latex-math/ml-boosting.tex <==
% ml - boosting
\newcommand{\fm}{f^{[m]}}                                                   % prediction in iteration m
\newcommand{\fmh}{\hat{f}^{[m]}}                                            % prediction in iteration m
\newcommand{\fmd}{f^{[m-1]}}                                                % prediction m-1
\newcommand{\fmdh}{\hat{f}^{[m-1]}}                                         % prediction m-1
\newcommand{\bmm}{b^{[m]}}                                                  % basemodel m
\newcommand{\bmmh}{\hat{b}^{[m]}}                                           % basemodel m with hat
\newcommand{\betam}{\beta^{[m]}}                                            % weight of basemodel m
\newcommand{\betamh}{\hat{\beta}^{[m]}}                                     % weight of basemodel m with hat
\newcommand{\betai}[1]{\beta^{[#1]}}                                        % weight of basemodel with argument for m
\newcommand{\errm}{\text{err}^{[m]}}                                        % weighted in-sample misclassification rate
\newcommand{\wm}{w^{[m]}}                                                   % weight vector of basemodel m
\newcommand{\wmi}{w^{[m](i)}}                                               % weight of obs i of basemodel m
\newcommand{\thetam}{\theta^{[m]}}                                          % parameters of basemodel m
\newcommand{\thetamh}{\hat{\theta}^{[m]}}                                   % parameters of basemodel m with hat
\newcommand{\rmm}{r^{[m]}}                                                  % pseudo residuals
\newcommand{\rmi}{r^{[m](i)}}                                               % pseudo residuals
\newcommand{\Rtm}{R_{t}^{[m]}}                                              % terminal-region
\newcommand{\Tm}{T^{[m]}}                                                   %
\newcommand{\ctm}{c_t^{[m]}}                                                % mean, terminal-regions
\newcommand{\ctmh}{\hat{c}_t^{[m]}}                                         % mean, terminal-regions with hat
\newcommand{\ctmt}{\tilde{c}_t^{[m]}}                                       % mean, terminal-regions
\newcommand{\fxk}{f_k(x)}                                                   % f_k(x)
\newcommand{\Lp}{L^\prime}
\newcommand{\Ldp}{L^{\prime\prime}}
\newcommand{\Lpleft}{\Lp_{\text{left}}}

==> latex-math/ml-gp.tex <==
% ml - Gaussian Process

\newcommand{\gp}{\mathcal{GP}\left(m(x), k\left(x, x'\right)\right)} 								% Gaussian Process Definition	
\newcommand{\mvec}{\bm{m}}												    						% Gaussian process mean vector
\newcommand{\Kmat}{\bm{K}}																			% estimated base learner 
\newcommand{\ls}{\ell}                                           % length-scale


==> latex-math/ml-mbo.tex <==
% ml - MBO
\newcommand{\sxh}{\hat{s}(x)} % uncertainty shat(x)
\newcommand{\vxh}{\hat{s}^2(x)}
\newcommand{\matK}{\mathbf{K}}
\newcommand{\kstarx}{\mathbf{k}_*(x)}
\newcommand{\xpi}[1][i]{x^{*(#1)}}
\newcommand{\vhx}{\ensuremath{\sh^2(\xv)}\xspace}          % local estimated variance at point x
\newcommand{\shx}{\ensuremath{\sh(\xv)}\xspace}            % local estimated uncertainty at point x
\newcommand{\sh}{\ensuremath{\hat{s}}\xspace}              % local estimated uncertainty
\newcommand{\px}{\ensuremath{\boldsymbol{x}^*}}
\newcommand{\equote}[1]{``#1''}
\newcommand{\vecx}{\ensuremath{\boldsymbol{x}}}
\newcommand{\yx}{\ensuremath{y(\vecx)}}
\newcommand{\X}{\ensuremath{\mathcal{X}}\xspace}           % domain / search space

% already defined in basic-math:
% \newcommand{\yv}{\boldsymbol{y}}
\newcommand{\fhx}{\ensuremath{\fh(\xv)}\xspace}            % surrogate (x), better use \mhx for predicted value

==> latex-math/ml-nn.tex <==
% ml - NNs
\newcommand{\neurons}{z_1,\dots,z_M} % vector of neurons

\newcommand{\hidz}{\mathbf{z}}                            % vector of hidden activations
\newcommand{\biasb}{\mathbf{b}}                           % bias vector
\newcommand{\wtw}{\mathbf{w}}                             % weight vector (general)
\newcommand{\wtu}{\mathbf{u}}                             % weight vector of output neuron
%


% deeplearning - regularization
\newcommand{\Oreg}{\mathnormal{R}_{reg}(\theta|X,y)}				% regularized objective function
\newcommand{\Ounreg}{\mathnormal{R}_{emp}(\theta|X,y)}			% unconstrained objective function
\newcommand{\Pen}{\Omega(\theta)}							% penalty
\newcommand{\Oregweight}{\mathnormal{R}_{reg}(w|X,y)}			% regularized objective function with weight 
\newcommand{\Oweight}{\mathnormal{R}_{emp}(w|X,y)}				% unconstrained objective function with weight
\newcommand{\Oweighti}{\mathnormal{R}_{emp}(w_i|X,y)}			% unconstrained objective function with weight w_i
\newcommand{\Oweightopt}{\mathnormal{J}(w^*|X,y)}				% unconstrained objective function withoptimal  weight
\newcommand{\Oopt}{\hat{\mathnormal{J}}(\theta|X,y)}				% optimal objective function 
\newcommand{\Odropout}{\mathnormal{J}(\theta, \mu|X,y)}	           	% dropout objective function

% deeplearning - optimization
\newcommand{\Lmomentum}{L(\yi, f(x^{(i)}, \theta + \varphi \nu))}                  % momentum risk

% deeplearning - autoencoders
\newcommand{\uauto}{L(x,g(f(x)))}			% undercomplete autoencoder objective function
\newcommand{\dauto}{L(x,g(f(\tilde{x})))}		% denoising autoencoder objective function


==> latex-math/ml-svm.tex <==
% ml - svms
\newcommand{\sv}{\operatorname{SV}}                                         % supportvectors
% already defined in basic-math:
% \newcommand{\HS}{\mathcal{H}}                                               % H, hilbertspace
\renewcommand{\sl}{\zeta}
\newcommand{\slvec}{\left(\zeta^{(1)}, \zeta^{(n)}\right)}		% slack variables (SVM)
\newcommand{\sli}{\zeta^{(i)}}																% slack variable (SVM)


==> latex-math/ml-trees.tex <==
% ml - trees, extra trees

\newcommand{\Np}{\mathcal{N}}												% (Parent) node N
\newcommand{\Nl}{\Np_1}														% Left node N_1
\newcommand{\Nr}{\Np_2}														% Right node N_2
\newcommand{\pikN}{\hat{\pi}_{\Np k}}             % estimated class probability in N

